An EMOF-Compliant Abstract Syntax for Bigraphs

Bigraphs are an emerging modeling formalism for structures in ubiquitous computing. Besides an algebraic notation, which can be adopted to provide an algebraic syntax for bigraphs, the bigraphical theory introduces a visual concrete syntax which is intuitive and unambiguous at the same time; the standard visual notation can be customized and thus tailored to domain-specific requirements. However, in contrast to modeling standards based on the Meta-Object Facility (MOF) and domain-specific languages typically used in model-driven engineering (MDE), the bigraphical theory lacks a precise definition of an abstract syntax for bigraphical modeling languages. As a consequence, available modeling and analysis tools use proprietary formats for representing bigraphs internally and persistently, which hampers the exchange of models across tool boundaries. Moreover, tools can be hardly integrated with standard MDE technologies in order to build sophisticated tool chains and modeling environments, as required for systematic engineering of large systems or fostering experimental work to evaluate the bigraphical theory in real-world applications. To overcome this situation, we propose an abstract syntax for bigraphs which is compliant to the Essential MOF (EMOF) standard defined by the Object Management Group (OMG). We use typed graphs as a formal underpinning of EMOF-based models and present a canonical mapping which maps bigraphs to typed graphs in a natural way. We also discuss application-specific variation points in the graph-based representation of bigraphs. Following standard techniques from software product line engineering, we present a framework to customize the graph-based representation to support a variety of application scenarios.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{Alexander Heu{\ss}ner, Aleks Kissinger, Anton Wijs (Eds.):\\ 2nd Graphs as Models workshop (GaM 2016)\\
EPTCS 231, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.231.2}{10.4204/EPTCS.231.2}}
\pdfoutput=1

